StyleGenes: Discrete and Efficient Latent Distributions for GANs

We propose a discrete latent distribution for Generative Adversarial Networks (GANs). Instead of drawing latent vectors from a continuous prior, we sample from a finite set of learnable latents. However, a direct parametrization of such a distribution leads to an intractable linear increase in memory in order to ensure sufficient sample diversity. We address this key issue by taking inspiration from the encoding of information in biological organisms. Instead of learning a separate latent vector for each sample, we split the latent space into a set of genes. For each gene, we train a small bank of gene variants. Thus, by independently sampling a variant for each gene and combining them into the final latent vector, our approach can represent a vast number of unique latent samples from a compact set of learnable parameters. Interestingly, our gene-inspired latent encoding allows for new and intuitive approaches to latent-space exploration, enabling conditional sampling from our unconditionally trained model. Moreover, our approach preserves state-of-the-art photo-realism while achieving better disentanglement than the widely-used StyleMapping network.

==> experiments.tex <==
\section{Experiments}\label{sec:experiments}

\textbf{Implementation}
Our method, StyleGenes, is written in Pytorch~\cite{pytorch}. We incorporate our sampling approach into two baseline models: (1) StyleGAN2~\cite{Karras2019stylegan2} as provided in the 
StyleGAN3~\cite{stylegan3Karras2021} codebase and ProjectedGANs~\cite{Sauer2021ProjectedGC} using the FastGAN~\cite{liu2021towards} generator. 
For all datasets, we train all our models and baselines \textit{unconditionally} using 4 GPUs following the default configuration as described in each project's code repository~\cite{stylegan3Karras2021,Sauer2021ProjectedGC}. For small datases Metfaces~\cite{Karras2020ada} and AFHQ~\cite{choi2020starganv2} we use adaptive discriminator augmentation~\cite{Karras2020ada}.
For our StyleGAN2 experiments, we train until the discriminator has seen 10 million images of resolution $256 \times 256$.
For ProjectedGAN, we train for their reported number of iterations to reach state-of-the-art results, rounded up to the next million: 8M images for FFHQ\cite{Karras_2019_CVPR} and 2M images for the other datasets. 

\textbf{Datasets}
We investigate the performance of our network using the \textit{Fr\'echet Inception Distance (FID)}~\cite{NIPS2017_7240}, on widely used datasets for unsupervised image generation:\\
\textbf{FFHQ}~\cite{Karras_2019_CVPR}, standing for Flickr Faces - High Quality is a collection of 70,000 face images scraped from flickr.com. The images were centered around the eyes and the mouth of the individual, offering strong position priors. The people depicted in the images come from a diverse background, age and poses.\\ 
\textbf{MetFaces}~\cite{Karras2020ada} is a dataset of image crops from art pieces of the Metropolitan Museum of Art Collection.
Similarly to FFHQ the crops are centered around human faces. 
The dataset contain 1336 images in total. The images are under CC0 license by the Metropolitan Museum of Art. Both FFHQ and Metfaces are licensed under CC BY-NC 2.0 license by NVIDIA Corp.\\
\textbf{AFHQ}~\cite{choi2020starganv2} is a collection of 15.000 images of animal faces divided equally into three categories: cat, dog and wildlife. However, in this work we do not use the labels for conditional generation. The dataset is available under CC BY-NC 4.0 license by NAVER Corp. 

\textbf{LSUN Church \& Bedroom}~\cite{yu15lsun}. We are using two subsets of the LSUN dataset \emph{Church} and \emph{Bedroom}, where they contain diverse outdoor and indoor scenes respectively. We use the full LSUN Church dataset of 126,227 images and a subset of the bedroom scenes comprised of 121,000 images. 


\subsection{Unconditional Generation}
In Table~\ref{tab:resablations}-left we can see the results obtained when introduce our discrete sampling technique to established baselines~\cite{Karras2019stylegan2, Sauer2021ProjectedGC}.
We compare them to the results we get when we train our baselines~\cite{Karras2020ada,Sauer2021ProjectedGC} with the same hyperparameters and training images,  
Our proposed discrete method produces similar results with StyleGAN's StyleMapping approach, and improves ProjectedGAN when it replaces gaussian sampling. 

In ablation study (Table~\ref{tab:resablations}-right), we aim to analyze the effect of the different Genome configurations to the perceptual performance of the network. 
Note that by keeping the number of the variants constant, the memory footprint of our approach is also constant.
Thus, every experiment that is in the same row in Table~\ref{tab:resablations}-right is using the same number of parameters that scale with the number of variants: $n_{v} * d$.
Increasing this number improves the perceptual quality in terms of FID, an effect more prominent for larger genes.
We call this an increase of \emph{parameter capacity}.
Alternatively, by increasing the number of genes, we also observe a decrease in FID.
Note that as we want to keep the size of the resulting latent vector constant $d=512$, we decrease each gene's length when using more. 
Therefore, the number of different images the genome can represent is also increasing, per Eq.~\eqref{eq:combo}.
We call this an increase of \emph{combinatorial capacity}.
Increasing the combinatorial capacity does not increase the parameters of the genome.
In Table~\ref{tab:resablations}-right we can observe that for all three datasets, for the smallest gene length, going from variants' number of $2048$ to $256$ leads to a minor deterioration of performance. However, the memory footprint of the genome is decreased 8-fold. 

\figDisentanglement{tab:disent}

\subsection{Analyzing the Codebook}

In this section we aim to analyze the properties that arise due to the discrete nature of our approach. Moreover, we show how to use them for conditional generation in FFHQ.

\textbf{Associating variants with attributes} 
As described in Section \ref{sec:method} we run a Monte Carlo experiment to estimate the probability $p(a_l | k_i=j)$ of the variant $j$ at position $i$ resulting to the attribute $a_l$ in the output image. 
We randomly sample $500,000$ gene sequences from our FFHQ model and generate their corresponding images.
We pass each of these images through 40 pretrained CelebA classifiers~\cite{celeba2015liu}.
Their weights are included in the original StyleGAN~\cite{Karras_2019_CVPR} code repository, and we used the code provided by StyleSpace~\cite{stylespaceWu2021} to extract the logits for every image.

\figConditional{fig:conditional}

\textbf{Conditional Generation}
In the previous step we acquired the marginal attribute distribution for a given genome variant. We use this information to conditionally generate an image with a desired attribute $a_l$. To generate unconditionally we sample the variant for each gene position uniformly. However, as described in Section \ref{sec:method} we can now infer the conditional latent distribution $p(k|{a_l})$ and use it to sample the variants instead. In Figure \ref{fig:conditional} we can see the results of our conditional sampling. Decreasing the temperature $t$ increases the likelihood of the presence of the desired attribute, however, can also limit the variability of the conditional outputs. This effect is outline in increased FID scores in Table \ref{fig:conditional} 

To gauge the ability of our method to generate conditionally, we train a conditional StyleGAN2 model with pseudo-labels from the CelebA classifiers. In Table \ref{fig:conditional}, we find we compare similarly to our baseline. However, we do not require a predefined number of classes and our method can be extended to more classes without training. Moreover, we can use the temperature value to control the trade-off between variability and accuracy.  
Lastly, training conditionally with a small dataset can lead to poor performance and mode collapse~\cite{shahbazi2022collapse}.

\textbf{Which genes are responsible for each attribute?}
We want to test if, like its biological inspiration, our genome has specific genes that control the expression of certain attributes, such as hair color.
We quantify this by calculating the \emph{mean absolute standard score} for each gene position: the absolute distance in terms of standard deviations that the gene variants have on average with the codebook's mean expected value for the particular attribute:
$s_{l}^{i} = \Sigma_{j}\frac{\lvert p(a_l| k_i=j) - \mu_{p(a_l| k_i)} \rvert}{\sigma_{p(a_l| k_i)}}$. 

In Figure~\ref{fig:analysis} we see the score for a gene in a specific position.
The genes are placed circularly around the plot.
Each color represents one of the 40 attributes.
Most genes do not significantly affect any of the attributes, instead controlling local image details. 
For each attribute, only a handful of genes have high standard scores.
On the right side of Figure~\ref{fig:analysis}, we see how changing the variants of specific genes alters the output image.
We sample a gene sequence and start substituting the variant of one gene at random. 
Manipulating the genes that exhibit high scores in the polar plot, such as genes 66, 85, and 38, leads to visible changes in the image.  


\figInterpolation{fig:interpolation}
\textbf{StyleGenome and Disentanglement}
The StyleGAN's~\cite{Karras_2019_CVPR} motivation to design the StyleMapping Network to make the sampling density determined by the mapping and not to be limited to any fixed distribution;
they aimed for the resulting space W to be more disentangled.
We explore how disentangled our \emph{StyleGenes} are compared to the output space of StyleMapping.
We train a Multi-Layer Perceptron to predict the presence of an attributed in an image from its latent code.
We randomly sample 50.000 codes from each of the two representations.
Then we extract the fake images' attributes using the pretrained classifiers, and appropriately prepared the train/val/test subsets.
We find that StyleGenes outperforms the StyleMapping's accuracy on every attribute we tested, with a ~10\% average increase, as shown in Table~\ref{tab:disent}-bottom.

\textbf{Interpolation}.
During training we sample the latent codes from our discrete codebook, but their values lie on $\mathbb{R}^d$.
We want to gauge whether the learned genome comprises samples that lie on a smooth surface. 
We sample two codes and interpolate between them. In Figure~\ref{fig:interpolation} we can see interpolation results for all three datasets.
The transition is smooth and the subsequent samples are semantically coherent and realistic.
By optimizing on discrete samples we are able to learn a continuous distribution.

\textbf{Adding real images in the codebook}.
We extend the Pivotal Tuning Inversion~\cite{roich2021pivotal} approach to project real images into our codebook in Figure \ref{fig:interpolation}. We start by concurrently optimizing a set of vectors in the underlying continuous space to produce the images we want to invert. Then, we find the indices of the nearest-neighbor variant for each gene position in the codebook. We  train both the generator and the codebook to recreate the images, based only on these indices. We substitute PTI's locality regularization with our codebook regularization: we push randomly sample gene-variants to keep their syntheses unchanged via an l2 and LPIPS~\cite{zhang2018perceptual} loss. We find this step important to retain the perceptual quality of the codebook.



==> limitations.tex <==
\section{Ethical Discussion}

Our methodology permits exploiting the discrete latent code of an image generator trained in an unsupervised manner, to generate conditionally and manipulate the output samples. However, it comes with some limitations.
First, while GANs aim to mimic the distribution of real images there is a gap between the real and fake distribution~\cite{precisionrecall}.
We apply a classifier trained on real images to infer the labels of fake images.
% In Figure~\ref{fig:conditional} we can see that the \emph{wearinghat} classifier gives the highest probability to erroneous samples, while we find more realistic hats in other rows.
The classifiers are limited by the entanglements of attributes in the training dataset. 
This issue is also discussed in StyleSpace~\cite{stylespaceWu2021}, where they note that the classifier may fail to predict a lipstick on a male face.
We hypothesize that this effect is further intensified because, while FFHQ offers significant diversity in ``age, ethnicity and accessories'', CelebA contains celebrity faces and thus is more limited in those factors.
% We hypothesize this is the reason that classifiers learned to associate.
Lastly, the biases of the labelers of the images can be propagated to the conditional image generation and manipulation results (See \emph{attractive} in Figure~\ref{fig:conditional}.
Therefore, one should be wary to apply this approach to a real life application.

Please not that in this work we train our model using portraits of real people, using the Flickr-Faces-HQ dataset~\cite{Karras_2019_CVPR}. As described in \emph{https://github.com/NVlabs/ffhq-dataset}, the images were collected to adhere to privacy rules and were filtered to only include samples intented for redistribution. Moreover, if an individual identifies themselves in the dataset, they can request the removal of their face from the collection.


==> source/changed_relatedwork.tex <==

\section{Related Work}

\noindent\textbf{Latent Code Quantization:}
VQ-VAE~\cite{VQVAEOord2017NeuralDR} is one of the first studies to exploit discrete representations for image generation,
designed to prevent the posterior collapse in VAE framework. % when the latent representations are paired with a powerful decoder.
% Instead of a continuous latent space, VQ-VAE represents the latent space as a spatial grid of quantized local latent codes, which are sampled from a discrete set of learned vectors in an auto-regressive manner.
VQ-VAE represents the latent space as a spatial grid of quantized local latent codes, which are sampled from a discrete set of learned vectors in an auto-regressive manner.
% VQ-VAE2~\cite{VQVAE2Razavi2019GeneratingDH} improving upon VQ-VAE, is capable of generating images of higher diversity and resolution by using a hierarchical multi-scale latent maps. 
VQ-VAE2~\cite{VQVAE2Razavi2019GeneratingDH} improves the image generation diversity and resolution by using hierarchical multi-scale latent maps. 
% The idea of VQ-VAE later on was extended to a GAN framework by changing the reconstruction loss and adding an adversarial one~\cite{VQGANEsser2021TamingTF}.
VQ-GAN extended the idea by changing the reconstruction loss and adding an adversarial one~\cite{VQGANEsser2021TamingTF}.
A transformer learns the auto-regressive priors for sampling the discrete local latent vector.
% The auto-regressive sampling of VQ-GANs~\cite{VQGANEsser2021TamingTF} for long sequences of discrete representations can be computationally inefficient.
% On the other hand, reducing the length of the sequences in VQ-VAE leads to performance degradation.
% Building on the previous approaches, 
RQ-VAE~\cite{lee2022autoregressive} proposes a residual feature quantization framework, which enables their model to work with smaller number of representation vectors.
Feature quantization has also been used in the discriminator of GANs to increase the stability of the adversarial training~\cite{pmlr-v119-zhao20d}.
Similarly to the above works we formulate the latent space as a composition of discrete feature vectors.
However, different to prior studies, we investigate discrete sampling of the latent code in the unsupervised GAN framework~\cite{Karras2019stylegan2}, without employing any encoder or self-supervised objective. 
% These approaches deploy an auto-encoder based approach, that produce local discrete codes and need auto-regressive sampling to draw new samples. 
These auto-encoder based approaches produce local discrete codes and need auto-regressive sampling to draw new samples. 
Our codebook is not trained through vector quantization, but rather through the adversarial game; it provides a global description of the image to be generated and thus does not require auto-regressive sampling.

\noindent\textbf{Latent code as a composition of smaller parts:}
InfoGAN~\cite{10.5555/3157096.3157340} aimed at increasing the interpretability and disentanglement of GANs' latent codes by maximizing the mutual information between parts of the latent and its corresponding images.
Inspired by the formation of DNA from genes, DNA-GAN~\cite{dnaganxiao2018} and ELEGANT~\cite{ElegantXiao2018} proposed dividing the latent code into smaller attribute-relevant and attribute-irrelevant parts, which are then supervised using attribute annotations to create attribute disentanglement in GANs. Similar to these studies, or method divides the style vectors into smaller codes. 
% Additionally, the style codes in our method consist of smaller codes.
However, 
% different to InfoGAN,
we only use a discrete set of codes to form the latent style codes. Note, we do not explicitly train our method for disentanglement and feature transfer but only for unconditional image synthesis.

\noindent\textbf{Analyzing the style space:}
Steering the latent space of GANs is paramount for image editing and conditional generation applications~\cite{jahanian2020steerability, yang2019semantic, voynov2020unsupervised}. Previous studies focus primarily on analyzing the style space, as it is more well-behaved and disentangled compared to the traditional latent space in prior GAN models. One goal of these analyses is to discover meaningful directions in the style space for semantic editing of images~\cite{stylespaceWu2021, jahanian2020steerability}. Moreover,~\cite{explaining_in_style} uses style space to explain and interpret the decisions made by attribute classifiers. The style space has also provided the opportunity for paired data generation using only a few annotations~\cite{zhang21}.
Recent methods utilize unconditionally pretrained models for conditional generation~\cite{styleflow, styleEMB_neurips2021}. These approaches, train a conditional normalizing flow~\cite{styleflow} or a classifier~\cite{styleEMB_neurips2021} in the latent space 
to enable conditional sampling.% Despite the extensive exploration, all of these methods focus on analyzing and steering a continuous style space.
% In this study, we analyze some of the characteristics of the newly proposed style space.
In this study, we do not need to train one vector per transformation~\cite{jahanian2020steerability}, compute any gradients\cite{stylespaceWu2021} or apply clustering to hidden layers~\cite{Collins2020EditingIS}. In contrast, we treat the network as a black box and, without extra training, only harness the benefits of its discrete input to enable conditional generation.  

% Note that we do not only provide alternative solutions for steering it for image editing, but also introduce a method for conditional generation.



